AIM: Accelerating Arbitrary-precision Integer Multiplication on Heterogeneous Reconfigurable Computing Platform Versal ACAP

Arbitrary-precision integer multiplication is the core kernel of many applications in simulation, cryptography, etc. Existing acceleration of arbitrary-precision integer multiplication includes CPUs, GPUs, FPGAs, and ASICs. Among these accelerators, FPGAs are promised to provide both good energy efficiency and flexibility. Surprisingly, in our implementations, FPGA has the lowest energy efficiency, i.e., 0.29x of the CPU and 0.17x of the GPU with the same generation fabrication. Therefore, key questions arise: Where do the energy efficiency gains of CPUs and GPUs come from? Can reconfigurable computing do better? If can, how to achieve that? We identify that the biggest energy efficiency gains of the CPUs and GPUs come from the dedicated vector units. FPGA uses DSPs and lookup tables to compose the needed computation, which incurs overhead when compared to using vector units directly. New reconfigurable computing, e.g., 'FPGA+vector units' is a novel and feasible solution to improve energy efficiency. In this paper, we propose to map arbitrary-precision integer multiplication onto such a heterogeneous platform, i.e., AMD/Xilinx Versal ACAP architecture. Designing on Versal ACAP incurs several challenges and we propose AIM: Arbitrary-precision Integer Multiplication on Versal ACAP to automate and optimize the design. AIM framework includes design space exploration and AIM automatic code generation to facilitate the system design and verification. We deploy the AIM framework on three different applications, including large integer multiplication (LIM), RSA, and Mandelbrot, on the AMD/Xilinx Versal ACAP VCK190 evaluation board. Our experimental results show that AIM achieves up to 12.6x, and 2.1x energy efficiency gains over the Intel Xeon Ice Lake 6346 CPU, and NVidia A5000 GPU respectively, which brings reconfigurable computing the most energy-efficient platform among CPUs and GPUs.

==> table/3_size_DSE.tex <==
% \begin{table}
% \caption{The highest achievable performance of AIM architecture for 1k bits multiplication predicted by AIM-DSE}

% \label{tbl:1kDSE}
% \begin{adjustbox}{width=\columnwidth,center}
% \begin{tabular}{ c | c | c | c | c }
% \toprule
%     Input Size & $P_{Intra}$ & $P_{Inter}$ & $PKT_{Ratio}$ & Performance (GOPs) \\
% \midrule
%    1,024 (Intra-only) & 20 & 1 & 0 & 11 \\
%    1,024 (Hybrid) & 40 & 3 & 0 & 31.5 \\
%    1,024 (Inter-only) & 1 & 32 & 0 & 113.92 \\
% \bottomrule

% \end{tabular}

% \end{adjustbox}
% \end{table}

% \begin{table}
% \caption{The highest achievable performance of AIM architecture for 32k bits multiplication predicted by AIM-DSE}

% \label{tbl:32kDSE}
% \begin{adjustbox}{width=\columnwidth,center}
% \begin{tabular}{ c | c | c | c | c }
% \toprule
%     Input Size & $P_{Intra}$ & $P_{Inter}$ & $PKT_{Ratio}$ & Performance (GOPs) \\
% \midrule
%    32,768 (Intra-only) & 272 & 1 & 0 & 1101 \\
%    32,768 (Hybrid) & 90 & 3 & 0 & 2456 \\
%    32,768 (Inter-only) & - & - & - & - \\
% \bottomrule

% \end{tabular}

% \end{adjustbox}
% \end{table}

% \begin{table}
% \caption{The highest achievable performance of AIM architecture for 512k bits multiplication predicted by AIM-DSE}

% \label{tbl:512kDSE}
% \begin{adjustbox}{width=\columnwidth,center}
% \begin{tabular}{ c | c | c | c | c }
% \toprule
%     Input Size & $P_{Intra}$ & $P_{Inter}$ & $PKT_{Ratio}$ & Performance (GOPs) \\
% \midrule
%    524,288 (Intra-only) & 306 & 1 & 0 & 3686.7 \\
%    524,288 (Hybrid) & - & - & - & - \\
%    524,288 (Inter-only) & - & - & - & - \\
% \bottomrule

% \end{tabular}

% \end{adjustbox}
% \end{table}


==> table/bandwidth.tex <==
\begin{table}
\caption{VCK190 I/O bandwdith and memory size.}
\vspace{-5pt}
\label{tbl:VCK190 I/O and Memory}
\begin{adjustbox}{width=\columnwidth,center}
%    \begin{center}
\begin{tabular}{ c  c | c  c}
    \toprule
    \multicolumn{2}{c|}{\textbf{I/O Bandwidth}} &
    \multicolumn{2}{c}{\textbf{Memory}}\\
    % \hline
   \textbf{Type}  &   \textbf{Perf(GB/s)}  &   \textbf{Type}  &   \textbf{Size(MB)}    \\
\midrule
   AIE $\leftrightarrow$AIE read/write   & 25600/12800  &   AIE array  &   12.5  \\
% \hline
  PL$\rightarrow$AIE / AIE$\rightarrow$PL   &  1248/936  &   PL (URAM+BRAM) &   20.5  \\
% \hline
   DDR$\leftrightarrow$PL   &  25.6  &  DIMM DDR4  &   8096   \\
    \bottomrule

\end{tabular}
 %   \end{center}
    \vspace{-10pt}
\end{adjustbox}
\end{table}

==> table/large_1kernel.tex <==
\begin{table}
\caption{Intra-Task Parallelism Single Kernel Performance}

\label{tbl:large_1kernel}
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{ c | c | c | c | c | c }
\toprule
    Input Size & Tile Size ($S$) & \#AIE  & PL Freq. (MHz) & Perf. (GOPs) \\
\midrule
   16,384 & 64 & 90 & {\color{red}xx} & {\color{red}xx} \\
   32,768 & 120 & 90 & {\color{red}xx} & {\color{red}xx} \\
   65,536 & 272 & 72 & {\color{red}xx} & {\color{red}xx} \\
   131,072 & 328 & 182 & {\color{red}xx} & {\color{red}xx} \\
   262,144 & 656 & 182 & {\color{red}xx} & {\color{red}xx} \\
   524,288 & 1,000 & 306 & 220 & 3,671 \\
\bottomrule

\end{tabular}

\end{adjustbox}
\end{table}


==> table/single_kernels_large.tex <==
\begin{table}
\caption{Intra-Task Parallelism Performance Scalling}

\label{tbl:large_perf}
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{ c | c | c | c | c | c }
\toprule
    Input Size & Tile Size ($S$) & \#AIE in 1PE & \#PE & PL Freq. (MHz) & Perf. (GOPs) \\
\midrule
   16,384 & 64 & 90 & 3 & 220 & 665 \\
   32,768 & 120 & 90 & 3 & 208 & 1,344 \\
   65,536 & 272 & 72 & 4 & 220 & 2,892 \\
   131,072 & 328 & 182 & 2 & 220 & 4,040 \\
   262,144 & 656 & 182 & 2 & 220 & 4,208 \\
   524,288 & 1,000 & 306 & 1 & 220 & 3,671 \\
\bottomrule

\end{tabular}

\end{adjustbox}
\end{table}


==> table/single_kernels_small.tex <==
% \begin{table}
% \caption{Inter-Task Parallelism Performance Scaling}

% \label{tbl:small_perf}
% \begin{adjustbox}{width=\columnwidth,center}
% \begin{tabular}{ c | c | c | c | c}
%     \toprule
%     Input Size & \#AIE used & $PKT_{ratio}$ & PL Freq. (MHz) & Perf. (GOPs) \\
% \midrule
%    512 & 32 & 0 & 224 & 31 \\
%    1,024 & 32 & 0 & 210 & 61 \\
%    2,048 & 32 & 0 & 196 & 119 \\
%    3,072 & 32 & 0 & {\color{red} xxx} & {\color{red} xxx} \\
%    4,096 & {\color{red} xxx} & 2 & {\color{red} xxx} & {\color{red} xxx} \\
%    8,192 & {\color{red} xxx} & 4 & {\color{red} xxx} & {\color{red} xxx} \\
%     \bottomrule

% \end{tabular}

% \end{adjustbox}
% \end{table}


==> table/small_1kernel.tex <==
% \begin{table}
% \caption{Inter-Task Parallelism Single Kernel Performance}

% \label{tbl:small_1kernel}
% \begin{adjustbox}{width=\columnwidth,center}
% \begin{tabular}{ c | c | c | c }
%     \toprule
%     Input Size & \#AIE used & PL Freq. (MHz) & Perf. (GOPs) \\
% \midrule
%    512 & 1 & 300 & 1.54 \\
%    1,024 & 1 & 300 & 3.56 \\
%    2,048 & 1 & 300 & 6.52 \\
%    3,072 & 1 & 300 & 8.39 \\
%    4,096 & 1 & 300 & 9.64 \\
%    8,192 & 1 & 300 & 11.5 \\
%     \bottomrule

% \end{tabular}

% \end{adjustbox}
% \end{table}

==> table/throughput_comparison.tex <==
\begin{table}[!tb]
\caption{Throughput Comparison}
\label{tbl:Throughput Comparison}
\begin{center}
\begin{adjustbox}{width=1\columnwidth,center}
\begin{tabular}{c | c | c | c | c | c | c | c}
\toprule
\textbf{Platforms}  & \textbf{CPU} &  \textbf{CPUAVX} &  \textbf{GPUV100} &  \textbf{GPUA5000} &  \textbf{FPGA} &  \textbf{ASIC} & \textbf{Versal ACAP}  \\ 
\midrule
Latency   & 88097   &  79866 &   1294   & 730  & 384 & 730  & 384 \\ 
Hardware Efficiency & 88097   &  79866 &   1294   & 730  & 384 & 730  & 384 \\ 
\bottomrule
\end{tabular}
\end{adjustbox}
\end{center}
\vspace{-20pt}
\end{table}
